Connections between Numerical Algorithms for PDEs and Neural Networks

We investigate numerous structural connections between numerical algorithms for partial differential equations (PDEs) and neural architectures. Our goal is to transfer the rich set of mathematical foundations from the world of PDEs to neural networks. Besides structural insights we provide concrete examples and experimental evaluations of the resulting architectures. Using the example of generalised nonlinear diffusion in 1D, we consider explicit schemes, acceleration strategies thereof, implicit schemes, and multigrid approaches. We connect these concepts to residual networks, recurrent neural networks, and U-net architectures. Our findings inspire a symmetric residual network design with provable stability guarantees and justify the effectiveness of skip connections in neural networks from a numerical perspective. Moreover, we present U-net architectures that implement multigrid techniques for learning efficient solutions of partial differential equation models, and motivate uncommon design choices such as trainable nonmonotone activation functions. Experimental evaluations show that the proposed architectures save half of the trainable parameters and can thus outperform standard ones with the same model complexity. Our considerations serve as a basis for explaining the success of popular neural architectures and provide a blueprint for developing new mathematically well-founded neural building blocks.

==> test_errors.tex <==
model modelid activation activationid coupling couplingid seed noise smoothness steps kernelsize channels parameters psnr mse
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 57360 10 5.0 1 3 1 8 32.08 40.30
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 57360 10 0.0 1 3 16 1568 34.73 21.88
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 57360 10 0.0 1 3 16 770 32.27 38.59
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 93840 10 5.0 1 3 1 9 33.88 26.63
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 93840 10 100000000.0 1 3 1 5 33.90 26.47
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 93840 10 100000000.0 1 3 1 5 33.67 27.91
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 93840 10 100000000.0 1 3 1 6 33.86 26.75
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 93840 10 100000000.0 1 3 1 4 31.58 45.21
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 93840 10 100000000.0 1 3 1 5 31.58 45.21
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 93840 10 10.0 1 3 1 5 33.90 26.47
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 93840 10 10.0 1 3 1 5 33.67 27.91
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 93840 10 10.0 1 3 1 6 33.86 26.75
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 93840 10 10.0 1 3 1 4 31.58 45.21
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 93840 10 10.0 1 3 1 5 31.58 45.21
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 93840 10 0.0 1 3 16 785 34.38 23.73
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 93840 10 0.0 1 3 16 786 34.38 23.73
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 93840 10 0.0 1 3 16 1584 34.70 22.05
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 93840 10 0.0 1 3 16 769 32.27 38.57
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 93840 10 0.0 1 3 16 785 34.10 25.30
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 93840 10 0.0 1 3 16 786 34.10 25.29
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 93840 10 0.0 1 3 16 770 32.27 38.57
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 15320 10 100000000.0 1 3 1 6 34.08 25.42
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 15320 10 10.0 1 3 1 6 34.08 25.42
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 15320 10 0.0 1 3 16 1584 34.72 21.93
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 15320 10 0.0 1 3 16 1584 34.70 22.05
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 72350 10 100000000.0 1 3 1 5 33.90 26.49
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 72350 10 100000000.0 1 3 1 5 33.67 27.96
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 72350 10 100000000.0 1 3 1 6 33.86 26.74
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 72350 10 10.0 1 3 1 5 33.90 26.49
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 72350 10 10.0 1 3 1 5 33.67 27.96
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 72350 10 10.0 1 3 1 6 33.86 26.74
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 12460 10 5.0 1 3 1 9 34.09 25.38
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 12460 10 100000000.0 1 3 1 5 33.90 26.47
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 12460 10 100000000.0 1 3 1 5 33.67 27.95
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 12460 10 100000000.0 1 3 1 6 33.86 26.76
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 12460 10 10.0 1 3 1 5 33.90 26.47
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 12460 10 10.0 1 3 1 5 33.67 27.95
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 12460 10 10.0 1 3 1 6 33.86 26.76
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 57360 10 100000000.0 1 3 1 8 32.08 40.30
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 93840 10 100000000.0 1 3 1 9 33.88 26.63
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 12460 10 100000000.0 1 3 1 9 34.09 25.38
FSI 3 CHARBONNIER 1 UNCOUPLED 1 93840 10 100000000.0 1 3 1 6 33.86 26.75
FSI 3 RELU 4 UNCOUPLED 1 93840 10 100000000.0 1 3 1 5 31.58 45.21
FSI 3 CHARBONNIER 1 UNCOUPLED 1 93840 10 10.0 1 3 1 6 33.86 26.75
FSI 3 RELU 4 UNCOUPLED 1 93840 10 10.0 1 3 1 5 31.58 45.21
FSI 3 PERONAMALIK 2 UNCOUPLED 1 93840 10 0.0 1 3 16 786 34.38 23.73
FSI 3 RELU 4 UNCOUPLED 1 93840 10 0.0 1 3 16 770 32.27 38.57
FSI 3 CHARBONNIER 1 UNCOUPLED 1 93840 10 0.0 1 3 16 786 34.10 25.30
FSI 3 PERONAMALIK 2 UNCOUPLED 1 72350 10 100000000.0 1 3 1 6 34.09 25.36
FSI 3 CHARBONNIER 1 UNCOUPLED 1 72350 10 100000000.0 1 3 1 6 33.86 26.74
FSI 3 PERONAMALIK 2 UNCOUPLED 1 72350 10 10.0 1 3 1 6 34.09 25.36
FSI 3 CHARBONNIER 1 UNCOUPLED 1 72350 10 10.0 1 3 1 6 33.86 26.74
FSI 3 PERONAMALIK 2 UNCOUPLED 1 12460 10 100000000.0 1 3 1 6 34.09 25.38
FSI 3 CHARBONNIER 1 UNCOUPLED 1 12460 10 100000000.0 1 3 1 6 33.86 26.76
FSI 3 PERONAMALIK 2 UNCOUPLED 1 12460 10 10.0 1 3 1 6 34.09 25.38
FSI 3 CHARBONNIER 1 UNCOUPLED 1 12460 10 10.0 1 3 1 6 33.86 26.76
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 40490 10 10.0 2 3 1 7 31.75 43.42
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 40490 10 0.0 2 3 16 3168 36.77 13.69
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 57360 10 0.0 2 3 16 3168 36.79 13.62
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 57360 10 0.0 2 3 16 3136 36.79 13.61
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 57360 10 0.0 2 3 16 1570 36.52 14.49
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 93840 10 5.0 2 3 1 16 32.28 38.48
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 93840 10 100000000.0 2 3 1 4 31.90 41.94
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 93840 10 100000000.0 2 3 1 5 32.02 40.82
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 93840 10 10.0 2 3 1 9 35.44 18.59
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 93840 10 10.0 2 3 1 10 35.25 19.43
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 93840 10 10.0 2 3 1 9 34.93 20.88
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 93840 10 10.0 2 3 1 10 34.77 21.70
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 93840 10 0.0 2 3 16 1570 36.67 13.99
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 93840 10 0.0 2 3 16 1569 36.63 14.13
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 15320 10 0.0 2 3 16 1538 36.27 15.33
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 72350 10 5.0 2 3 1 18 35.58 18.00
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 72350 10 5.0 2 3 1 18 35.05 20.31
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 72350 10 100000000.0 2 3 1 6 35.19 19.71
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 72350 10 100000000.0 2 3 1 5 34.61 22.52
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 72350 10 100000000.0 2 3 1 6 34.74 21.85
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 72350 10 10.0 2 3 1 8 31.96 41.40
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 72350 10 0.0 2 3 16 1569 36.51 14.53
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 72350 10 0.0 2 3 16 1537 36.18 15.67
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 12460 10 5.0 2 3 1 18 35.58 17.97
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 12460 10 5.0 2 3 1 18 35.05 20.33
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 12460 10 100000000.0 2 3 1 5 35.01 20.53
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 12460 10 100000000.0 2 3 1 6 35.19 19.70
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 57360 10 100000000.0 2 3 1 8 32.17 39.49
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 93840 10 100000000.0 2 3 1 9 35.06 20.29
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 12460 10 100000000.0 2 3 1 9 35.45 18.53
FSI 3 RELU 4 UNCOUPLED 1 57360 10 10.0 2 3 1 9 32.07 40.35
FSI 3 PERONAMALIK 2 UNCOUPLED 1 57360 10 0.0 2 3 16 1571 36.51 14.53
FSI 3 RELU 4 UNCOUPLED 1 93840 10 100000000.0 2 3 1 6 32.02 40.82
FSI 3 CHARBONNIER 1 UNCOUPLED 1 93840 10 10.0 2 3 1 11 34.95 20.83
FSI 3 PERONAMALIK 2 UNCOUPLED 1 93840 10 0.0 2 3 16 1571 36.51 14.54
FSI 3 CHARBONNIER 1 UNCOUPLED 1 93840 10 0.0 2 3 16 1571 36.66 14.02
FSI 3 RELU 4 UNCOUPLED 1 15320 10 0.0 2 3 16 1539 36.27 15.36
FSI 3 CHARBONNIER 1 UNCOUPLED 1 15320 10 0.0 2 3 16 1571 36.66 14.02
FSI 3 PERONAMALIK 2 UNCOUPLED 1 72350 10 100000000.0 2 3 1 7 35.40 18.75
FSI 3 CHARBONNIER 1 UNCOUPLED 1 72350 10 100000000.0 2 3 1 7 34.90 21.03
FSI 3 PERONAMALIK 2 UNCOUPLED 1 72350 10 10.0 2 3 1 11 35.57 18.04
FSI 3 CHARBONNIER 1 UNCOUPLED 1 72350 10 10.0 2 3 1 11 34.95 20.80
FSI 3 PERONAMALIK 2 UNCOUPLED 1 72350 10 0.0 2 3 16 1571 36.51 14.52
FSI 3 CHARBONNIER 1 UNCOUPLED 1 72350 10 0.0 2 3 16 1571 36.66 14.03
FSI 3 PERONAMALIK 2 UNCOUPLED 1 12460 10 100000000.0 2 3 1 7 35.40 18.74
FSI 3 CHARBONNIER 1 UNCOUPLED 1 12460 10 100000000.0 2 3 1 7 34.90 21.04
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 40490 10 0.0 3 3 16 4752 37.75 10.91
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 40490 10 0.0 3 3 16 2353 37.56 11.39
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 40490 10 0.0 3 3 16 2354 37.61 11.27
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 58210 10 10.0 3 3 1 11 31.89 42.05
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 58210 10 0.0 3 3 16 2354 37.42 11.79
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 12380 10 0.0 3 3 16 4752 37.75 10.93
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 57360 10 10.0 3 3 1 13 36.14 15.83
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 57360 10 10.0 3 3 1 14 35.95 16.52
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 57360 10 0.0 3 3 16 4704 37.74 10.93
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 93840 10 5.0 3 3 1 27 35.53 18.18
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 93840 10 100000000.0 3 3 1 4 31.84 42.61
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 93840 10 100000000.0 3 3 1 5 31.87 42.32
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 93840 10 10.0 3 3 1 14 35.95 16.53
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 93840 10 10.0 3 3 1 13 35.45 18.56
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 93840 10 10.0 3 3 1 14 35.29 19.22
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 93840 10 0.0 3 3 16 2354 37.61 11.26
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 83540 10 10.0 3 3 1 10 31.70 43.93
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 83540 10 0.0 3 3 16 2305 37.16 12.52
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 15320 10 5.0 3 3 1 24 32.31 38.17
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 72350 10 5.0 3 3 1 27 36.51 14.54
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 72350 10 100000000.0 3 3 1 6 35.87 16.83
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 72350 10 100000000.0 3 3 1 5 35.06 20.28
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 72350 10 100000000.0 3 3 1 6 35.24 19.47
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 72350 10 10.0 3 3 1 14 35.95 16.54
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 72350 10 10.0 3 3 1 13 35.45 18.56
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 72350 10 0.0 3 3 16 2353 37.46 11.68
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 72350 10 0.0 3 3 16 4752 37.75 10.93
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 72350 10 0.0 3 3 16 2306 37.24 12.29
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 12460 10 100000000.0 3 3 1 5 35.59 17.97
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 12460 10 100000000.0 3 3 1 6 35.87 16.83
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 12460 10 100000000.0 3 3 1 5 35.06 20.30
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 12460 10 10.0 3 3 1 10 31.70 44.00
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 57360 10 100000000.0 3 3 1 8 32.19 39.29
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 93840 10 100000000.0 3 3 1 9 35.51 18.27
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 12460 10 100000000.0 3 3 1 9 36.00 16.33
FSI 3 CHARBONNIER 1 UNCOUPLED 1 40490 10 0.0 3 3 16 2356 37.63 11.23
FSI 3 PERONAMALIK 2 UNCOUPLED 1 40490 10 0.0 3 3 16 2356 37.60 11.29
FSI 3 RELU 4 UNCOUPLED 1 57360 10 0.0 3 3 16 2308 37.18 12.44
FSI 3 RELU 4 UNCOUPLED 1 93840 10 100000000.0 3 3 1 7 32.24 38.82
FSI 3 RELU 4 UNCOUPLED 1 83540 10 10.0 3 3 1 13 32.86 33.70
FSI 3 PERONAMALIK 2 UNCOUPLED 1 72350 10 100000000.0 3 3 1 8 35.96 16.50
FSI 3 CHARBONNIER 1 UNCOUPLED 1 72350 10 100000000.0 3 3 1 8 35.36 18.91
FSI 3 PERONAMALIK 2 UNCOUPLED 1 72350 10 10.0 3 3 1 16 36.21 15.58
FSI 3 CHARBONNIER 1 UNCOUPLED 1 72350 10 10.0 3 3 1 16 35.52 18.25
FSI 3 PERONAMALIK 2 UNCOUPLED 1 12460 10 100000000.0 3 3 1 8 35.96 16.48
FSI 3 CHARBONNIER 1 UNCOUPLED 1 12460 10 100000000.0 3 3 1 8 35.36 18.92
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 58210 10 10.0 4 3 1 13 31.79 43.07
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 58210 10 0.0 4 3 16 3138 38.17 9.91
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 57360 10 10.0 4 3 1 18 35.69 17.55
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 57360 10 0.0 4 3 16 6272 38.35 9.50
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 57360 10 0.0 4 3 16 3074 37.81 10.78
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 93840 10 5.0 4 3 1 36 36.62 14.17
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 93840 10 5.0 4 3 1 36 35.80 17.10
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 93840 10 100000000.0 4 3 1 4 31.87 42.32
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 93840 10 100000000.0 4 3 1 5 32.06 40.44
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 93840 10 10.0 4 3 1 14 32.09 40.15
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 93840 10 0.0 4 3 16 3138 38.04 10.22
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 15320 10 5.0 4 3 1 32 32.32 38.12
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 15320 10 0.0 4 3 16 3073 37.80 10.80
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 72350 10 100000000.0 4 3 1 6 36.18 15.68
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 72350 10 100000000.0 4 3 1 5 35.33 19.07
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 72350 10 100000000.0 4 3 1 6 35.53 18.19
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 72350 10 10.0 4 3 1 17 36.58 14.31
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 72350 10 10.0 4 3 1 18 36.44 14.75
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 72350 10 10.0 4 3 1 17 35.72 17.43
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 72350 10 10.0 4 3 1 18 35.69 17.53
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 72350 10 0.0 4 3 16 6336 38.39 9.42
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 72350 10 0.0 4 3 16 3137 38.00 10.31
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 72350 10 0.0 4 3 16 6336 38.40 9.40
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 72350 10 0.0 4 3 16 3137 38.11 10.06
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 12460 10 100000000.0 4 3 1 5 35.93 16.61
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 12460 10 100000000.0 4 3 1 6 36.18 15.66
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 12460 10 100000000.0 4 3 1 6 35.53 18.21
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 12460 10 10.0 4 3 1 18 35.69 17.56
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 57360 10 100000000.0 4 3 1 8 32.20 39.20
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 93840 10 100000000.0 4 3 1 9 35.75 17.31
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 12460 10 100000000.0 4 3 1 9 36.30 15.25
FSI 3 PERONAMALIK 2 UNCOUPLED 1 93840 10 100000000.0 4 3 1 9 36.24 15.46
FSI 3 RELU 4 UNCOUPLED 1 93840 10 100000000.0 4 3 1 8 32.08 40.30
FSI 3 PERONAMALIK 2 UNCOUPLED 1 93840 10 10.0 4 3 1 21 36.74 13.79
FSI 3 RELU 4 UNCOUPLED 1 83540 10 100000000.0 4 3 1 8 32.08 40.32
FSI 3 RELU 4 UNCOUPLED 1 15320 10 10.0 4 3 1 17 33.22 30.97
FSI 3 RELU 4 UNCOUPLED 1 15320 10 0.0 4 3 16 3077 37.82 10.74
FSI 3 CHARBONNIER 1 UNCOUPLED 1 15320 10 0.0 4 3 16 3141 38.08 10.12
FSI 3 CHARBONNIER 1 UNCOUPLED 1 72350 10 100000000.0 4 3 1 9 35.63 17.80
FSI 3 PERONAMALIK 2 UNCOUPLED 1 72350 10 10.0 4 3 1 21 36.74 13.78
FSI 3 CHARBONNIER 1 UNCOUPLED 1 72350 10 10.0 4 3 1 21 35.85 16.92
FSI 3 PERONAMALIK 2 UNCOUPLED 1 72350 10 0.0 4 3 16 3141 38.22 9.80
FSI 3 CHARBONNIER 1 UNCOUPLED 1 72350 10 0.0 4 3 16 3141 38.08 10.12
FSI 3 PERONAMALIK 2 UNCOUPLED 1 12460 10 100000000.0 4 3 1 9 36.24 15.45
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 40490 10 100000000.0 5 3 1 6 36.55 14.38
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 40490 10 0.0 5 3 16 7920 38.83 8.52
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 12380 10 0.0 5 3 16 3922 38.60 8.97
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 57360 10 0.0 5 3 16 3921 38.44 9.31
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 57360 10 0.0 5 3 16 3841 38.23 9.77
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 57360 10 0.0 5 3 16 7840 38.73 8.71
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 57360 10 0.0 5 3 16 3842 38.30 9.62
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 93840 10 5.0 5 3 1 45 36.82 13.52
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 93840 10 5.0 5 3 1 45 35.99 16.38
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 93840 10 100000000.0 5 3 1 4 31.88 42.15
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 93840 10 100000000.0 5 3 1 5 31.91 41.88
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 93840 10 10.0 5 3 1 21 35.91 16.68
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 93840 10 10.0 5 3 1 22 35.92 16.64
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 93840 10 10.0 5 3 1 16 31.87 42.28
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 93840 10 10.0 5 3 1 17 31.96 41.37
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 15320 10 5.0 5 3 1 40 32.33 38.06
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 15320 10 10.0 5 3 1 17 31.96 41.42
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 15320 10 0.0 5 3 16 3921 38.51 9.17
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 15320 10 0.0 5 3 16 3922 38.62 8.93
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 72350 10 100000000.0 5 3 1 5 35.51 18.30
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 72350 10 100000000.0 5 3 1 6 35.77 17.24
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 72350 10 10.0 5 3 1 21 36.83 13.48
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 72350 10 10.0 5 3 1 22 36.72 13.83
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 72350 10 0.0 5 3 16 7920 38.83 8.51
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 12460 10 100000000.0 5 3 1 5 36.13 15.85
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 40490 10 100000000.0 5 3 1 9 36.59 14.26
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 57360 10 100000000.0 5 3 1 8 32.20 39.14
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 12460 10 100000000.0 5 3 1 9 35.88 16.80
FSI 3 PERONAMALIK 2 UNCOUPLED 1 40490 10 100000000.0 5 3 1 10 36.62 14.16
FSI 3 CHARBONNIER 1 UNCOUPLED 1 58210 10 0.0 5 3 16 3926 38.53 9.13
FSI 3 PERONAMALIK 2 UNCOUPLED 1 57360 10 10.0 5 3 1 26 37.01 12.94
FSI 3 PERONAMALIK 2 UNCOUPLED 1 93840 10 100000000.0 5 3 1 10 36.62 14.16
FSI 3 RELU 4 UNCOUPLED 1 83540 10 100000000.0 5 3 1 9 32.16 39.59
FSI 3 RELU 4 UNCOUPLED 1 83540 10 10.0 5 3 1 21 33.62 28.25
FSI 3 RELU 4 UNCOUPLED 1 15320 10 0.0 5 3 16 3846 38.23 9.78
FSI 3 PERONAMALIK 2 UNCOUPLED 1 15320 10 0.0 5 3 16 3926 38.69 8.80
FSI 3 CHARBONNIER 1 UNCOUPLED 1 72350 10 100000000.0 5 3 1 10 35.85 16.89
FSI 3 PERONAMALIK 2 UNCOUPLED 1 72350 10 10.0 5 3 1 26 37.01 12.93
FSI 3 CHARBONNIER 1 UNCOUPLED 1 72350 10 10.0 5 3 1 26 36.41 14.86
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 40490 10 100000000.0 7 3 1 6 37.00 12.96
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 58210 10 0.0 7 3 16 5489 39.19 7.84
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 57360 10 10.0 7 3 1 29 37.08 12.74
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 57360 10 10.0 7 3 1 30 37.11 12.65
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 57360 10 10.0 7 3 1 23 31.93 41.75
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 57360 10 0.0 7 3 16 5490 38.93 8.33
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 93840 10 5.0 7 3 1 56 32.37 37.68
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 93840 10 5.0 7 3 1 63 37.06 12.79
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 93840 10 5.0 7 3 1 63 36.18 15.69
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 93840 10 100000000.0 7 3 1 4 31.90 41.97
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 93840 10 10.0 7 3 1 22 31.91 41.90
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 93840 10 10.0 7 3 1 23 31.93 41.68
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 93840 10 0.0 7 3 16 5489 39.18 7.85
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 15320 10 5.0 7 3 1 63 37.06 12.81
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 15320 10 0.0 7 3 16 10976 39.35 7.56
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 15320 10 0.0 7 3 16 5378 38.84 8.50
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 72350 10 100000000.0 7 3 1 5 35.76 17.28
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 72350 10 100000000.0 7 3 1 6 36.08 16.05
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 72350 10 10.0 7 3 1 29 36.06 16.11
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 72350 10 0.0 7 3 16 11088 39.49 7.32
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 72350 10 0.0 7 3 16 11088 39.58 7.16
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 72350 10 0.0 7 3 16 10976 39.35 7.55
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 72350 10 0.0 7 3 16 5377 38.79 8.58
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 72350 10 0.0 7 3 16 5490 39.04 8.11
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 12460 10 100000000.0 7 3 1 5 36.51 14.54
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 12460 10 100000000.0 7 3 1 5 31.76 43.36
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 12460 10 10.0 7 3 1 30 37.11 12.66
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 12460 10 10.0 7 3 1 30 36.13 15.84
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 40490 10 100000000.0 7 3 1 9 36.95 13.13
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 58210 10 100000000.0 7 3 1 9 36.07 16.09
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 57360 10 100000000.0 7 3 1 8 32.21 39.09
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 12460 10 100000000.0 7 3 1 9 36.07 16.06
FSI 3 PERONAMALIK 2 UNCOUPLED 1 40490 10 100000000.0 7 3 1 12 37.06 12.80
FSI 3 RELU 4 UNCOUPLED 1 40490 10 10.0 7 3 1 29 34.28 24.29
FSI 3 CHARBONNIER 1 UNCOUPLED 1 40490 10 0.0 7 3 16 5496 39.15 7.90
FSI 3 RELU 4 UNCOUPLED 1 12380 10 0.0 7 3 16 5384 38.78 8.61
FSI 3 CHARBONNIER 1 UNCOUPLED 1 57360 10 10.0 7 3 1 36 37.02 12.91
FSI 3 RELU 4 UNCOUPLED 1 93840 10 100000000.0 7 3 1 11 32.25 38.76
FSI 3 RELU 4 UNCOUPLED 1 83540 10 0.0 7 3 16 5384 38.78 8.61
FSI 3 CHARBONNIER 1 UNCOUPLED 1 72350 10 100000000.0 7 3 1 12 36.14 15.83
FSI 3 PERONAMALIK 2 UNCOUPLED 1 72350 10 0.0 7 3 16 5496 39.24 7.75
FSI 3 PERONAMALIK 2 UNCOUPLED 1 12460 10 10.0 7 3 1 36 37.20 12.39
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 40490 10 5.0 10 3 1 90 37.21 12.36
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 40490 10 100000000.0 10 3 1 6 37.21 12.36
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 40490 10 10.0 10 3 1 41 37.20 12.40
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 40490 10 10.0 10 3 1 42 37.27 12.21
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 58210 10 5.0 10 3 1 80 32.45 37.04
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 58210 10 0.0 10 3 16 7681 39.38 7.50
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 58210 10 0.0 10 3 16 7842 39.72 6.94
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 57360 10 10.0 10 3 1 41 37.20 12.40
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 57360 10 10.0 10 3 1 42 37.27 12.18
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 57360 10 0.0 10 3 16 7682 39.26 7.71
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 93840 10 10.0 10 3 1 31 31.88 42.20
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 93840 10 10.0 10 3 1 32 32.74 34.60
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 83540 10 5.0 10 3 1 90 36.42 14.83
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 83540 10 0.0 10 3 16 7842 39.72 6.95
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 15320 10 0.0 10 3 16 7841 39.87 6.70
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 72350 10 100000000.0 10 3 1 5 36.02 16.28
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 72350 10 100000000.0 10 3 1 6 36.27 15.35
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 72350 10 0.0 10 3 16 15840 40.14 6.29
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 72350 10 0.0 10 3 16 7841 39.90 6.66
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 72350 10 0.0 10 3 16 15840 40.16 6.27
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 72350 10 0.0 10 3 16 15680 40.01 6.49
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 72350 10 0.0 10 3 16 7842 39.76 6.87
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 12460 10 100000000.0 10 3 1 5 36.89 13.32
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 12460 10 100000000.0 10 3 1 4 31.75 43.46
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 12460 10 100000000.0 10 3 1 5 31.86 42.35
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 12460 10 10.0 10 3 1 41 36.17 15.71
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 12460 10 10.0 10 3 1 42 36.29 15.28
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 40490 10 100000000.0 10 3 1 9 37.16 12.50
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 57360 10 100000000.0 10 3 1 8 32.22 39.05
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 12460 10 100000000.0 10 3 1 9 36.20 15.61
FSI 3 PERONAMALIK 2 UNCOUPLED 1 40490 10 100000000.0 10 3 1 15 37.23 12.30
FSI 3 CHARBONNIER 1 UNCOUPLED 1 40490 10 0.0 10 3 16 7851 39.77 6.86
FSI 3 RELU 4 UNCOUPLED 1 58210 10 10.0 10 3 1 41 34.23 24.55
FSI 3 RELU 4 UNCOUPLED 1 58210 10 0.0 10 3 16 7691 39.30 7.64
FSI 3 RELU 4 UNCOUPLED 1 93840 10 100000000.0 10 3 1 14 32.11 39.97
FSI 3 PERONAMALIK 2 UNCOUPLED 1 83540 10 0.0 10 3 16 7851 39.82 6.78
FSI 3 PERONAMALIK 2 UNCOUPLED 1 15320 10 10.0 10 3 1 51 37.42 11.78
FSI 3 CHARBONNIER 1 UNCOUPLED 1 72350 10 100000000.0 10 3 1 15 36.30 15.25
FSI 3 CHARBONNIER 1 UNCOUPLED 1 12460 10 10.0 10 3 1 51 37.25 12.24
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 40490 10 5.0 15 3 1 135 37.25 12.24
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 40490 10 100000000.0 15 3 1 5 37.15 12.54
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 40490 10 100000000.0 15 3 1 6 37.22 12.34
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 40490 10 10.0 15 3 1 62 37.30 12.12
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 40490 10 10.0 15 3 1 62 36.35 15.08
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 40490 10 0.0 15 3 16 11762 40.52 5.77
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 57360 10 10.0 15 3 1 61 37.26 12.21
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 57360 10 10.0 15 3 1 47 32.30 38.33
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 93840 10 10.0 15 3 1 46 31.81 42.86
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 15320 10 5.0 15 3 1 120 32.34 37.97
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 15320 10 0.0 15 3 16 23760 40.56 5.72
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 15320 10 0.0 15 3 16 11521 39.88 6.68
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 72350 10 5.0 15 3 1 135 36.97 13.05
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 72350 10 100000000.0 15 3 1 5 36.21 15.57
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 72350 10 100000000.0 15 3 1 6 36.32 15.18
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 72350 10 0.0 15 3 16 23760 40.70 5.54
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 72350 10 0.0 15 3 16 11761 40.50 5.79
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 72350 10 0.0 15 3 16 23520 40.32 6.04
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 72350 10 0.0 15 3 16 11761 40.55 5.73
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 72350 10 0.0 15 3 16 11522 39.89 6.67
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 12460 10 100000000.0 15 3 1 5 37.15 12.53
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 12460 10 100000000.0 15 3 1 4 31.76 43.37
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 12460 10 100000000.0 15 3 1 5 31.78 43.22
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 12460 10 10.0 15 3 1 61 36.26 15.37
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 12460 10 0.0 15 3 16 11762 40.08 6.39
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 40490 10 100000000.0 15 3 1 9 37.23 12.30
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 58210 10 100000000.0 15 3 1 9 36.26 15.39
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 57360 10 100000000.0 15 3 1 8 32.22 39.01
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 12460 10 100000000.0 15 3 1 9 36.26 15.37
FSI 3 PERONAMALIK 2 UNCOUPLED 1 40490 10 100000000.0 15 3 1 20 37.26 12.23
FSI 3 PERONAMALIK 2 UNCOUPLED 1 58210 10 10.0 15 3 1 76 37.51 11.55
FSI 3 CHARBONNIER 1 UNCOUPLED 1 12380 10 0.0 15 3 16 11776 39.52 7.25
FSI 3 RELU 4 UNCOUPLED 1 57360 10 10.0 15 3 1 61 34.91 20.99
FSI 3 RELU 4 UNCOUPLED 1 93840 10 100000000.0 15 3 1 19 32.25 38.76
FSI 3 RELU 4 UNCOUPLED 1 15320 10 0.0 15 3 16 11536 39.84 6.75
FSI 3 CHARBONNIER 1 UNCOUPLED 1 72350 10 100000000.0 15 3 1 20 36.33 15.14
FSI 3 PERONAMALIK 2 UNCOUPLED 1 72350 10 0.0 15 3 16 11776 40.45 5.87
FSI 3 CHARBONNIER 1 UNCOUPLED 1 12460 10 10.0 15 3 1 76 37.52 11.52
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 40490 10 100000000.0 20 3 1 5 37.21 12.38
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 40490 10 100000000.0 20 3 1 6 37.22 12.34
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 40490 10 10.0 20 3 1 82 37.29 12.15
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 58210 10 0.0 20 3 16 15681 40.44 5.88
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 12380 10 0.0 20 3 16 15682 40.16 6.27
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 57360 10 10.0 20 3 1 81 37.29 12.13
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 57360 10 10.0 20 3 1 82 37.29 12.14
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 93840 10 10.0 20 3 1 61 31.81 42.90
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 93840 10 0.0 20 3 16 31360 40.63 5.63
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 83540 10 10.0 20 3 1 62 32.53 36.31
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 15320 10 5.0 20 3 1 160 32.34 37.95
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 15320 10 0.0 20 3 16 31680 41.06 5.10
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 15320 10 0.0 20 3 16 15681 40.88 5.31
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 15320 10 0.0 20 3 16 31680 40.70 5.53
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 72350 10 5.0 20 3 1 180 37.07 12.77
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 72350 10 5.0 20 3 1 180 37.29 12.13
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 15320 10 0.0 20 3 16 15362 40.11 6.34
STABLE_RESNET 1 PERONAMALIK 2 UNCOUPLED 1 72350 10 100000000.0 20 3 1 5 37.21 12.35
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 72350 10 100000000.0 20 3 1 5 36.28 15.32
DUFORTFRANKEL 2 PERONAMALIK 2 UNCOUPLED 1 72350 10 100000000.0 20 3 1 6 37.22 12.32
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 72350 10 100000000.0 20 3 1 6 36.32 15.18
STABLE_RESNET 1 CHARBONNIER 1 UNCOUPLED 1 72350 10 10.0 20 3 1 81 36.30 15.26
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 72350 10 10.0 20 3 1 82 36.34 15.10
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 72350 10 0.0 20 3 16 15361 40.04 6.44
DUFORTFRANKEL 2 CHARBONNIER 1 UNCOUPLED 1 72350 10 0.0 20 3 16 15682 39.99 6.51
STABLE_RESNET 1 RELU 4 UNCOUPLED 1 12460 10 100000000.0 20 3 1 4 31.77 43.32
DUFORTFRANKEL 2 RELU 4 UNCOUPLED 1 12460 10 100000000.0 20 3 1 5 31.83 42.73
STANDARD_RESNET 0 PERONAMALIK 2 UNCOUPLED 1 40490 10 100000000.0 20 3 1 9 37.23 12.30
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 58210 10 100000000.0 20 3 1 9 36.28 15.33
STANDARD_RESNET 0 RELU 4 UNCOUPLED 1 57360 10 100000000.0 20 3 1 8 32.22 38.99
STANDARD_RESNET 0 CHARBONNIER 1 UNCOUPLED 1 12460 10 100000000.0 20 3 1 9 36.28 15.30
FSI 3 PERONAMALIK 2 UNCOUPLED 1 40490 10 100000000.0 20 3 1 25 37.26 12.23
FSI 3 CHARBONNIER 1 UNCOUPLED 1 40490 10 10.0 20 3 1 101 37.56 11.41
FSI 3 RELU 4 UNCOUPLED 1 58210 10 10.0 20 3 1 81 35.40 18.77
FSI 3 CHARBONNIER 1 UNCOUPLED 1 58210 10 0.0 20 3 16 15701 39.87 6.69
FSI 3 RELU 4 UNCOUPLED 1 93840 10 100000000.0 20 3 1 24 32.25 38.77
FSI 3 CHARBONNIER 1 UNCOUPLED 1 72350 10 100000000.0 20 3 1 25 36.33 15.14
FSI 3 PERONAMALIK 2 UNCOUPLED 1 72350 10 10.0 20 3 1 101 37.60 11.30
FSI 3 RELU 4 UNCOUPLED 1 15320 10 0.0 20 3 16 15381 40.10 6.36
FSI 3 PERONAMALIK 2 UNCOUPLED 1 15320 10 0.0 20 3 16 15701 40.59 5.68
CLASSICAL 4 PERONAMALIK 2 UNCOUPLED 1 40490 10 100000000.0 40 3 1 2 37.22 12.34
CLASSICAL 4 CHARBONNIER 1 UNCOUPLED 1 40490 10 100000000.0 40 3 1 2 36.25 15.43
CLASSICAL 4 ID 0 UNCOUPLED 1 57360 10 100000000.0 40 3 1 1 31.20 49.28

